Studies on Generalized Warped Five-Dimensional Models

In this thesis we study a number of aspects about warped five-dimensional models. We first discuss on the construction of soft-wall models. We provide recipes for constructing consistent models of this kind and address the issue of how the length of the extra dimension can be stabilized. We also discuss on the spectrum of fluctuations that arise in soft-wall models and we present a concrete model where a large UV/IR hierarchy can be generated without any fine-tuning. Next, we consider a two-brane setup to study how the electroweak symmetry can be broken in warped models with generalized metrics when the Higgs boson propagates in the bulk. We show how the bounds on the Kaluza-Klein (KK) scale that arise from electroweak precision observables can be alleviated when the Higgs is localized towards the infrared brane. We apply our results to a minimal 5D extension of the SM and consider the AdS geometry and a deformation of it inspired by soft-walls. We find that the deformed geometry greatly reduces the bounds on the KK scale, to a point where the KK states can be within the range of the LHC and the little hierarchy problem can be removed without requiring the introduction of any custodial symmetry. Finally, we study the propagation of all SM fermions in the bulk of the extra dimension, which we use to address the flavor puzzle of the SM. We find general explicit expressions for oblique and non-oblique electroweak observables, as well as flavor and CP violating operators. We apply these results to the RS model and the model with deformed geometry, for which we perform a statistical analysis departing from a random set of 5D Yukawa couplings. The comparison of the predictions with the current experimental data exhibits an improvement of the bounds in our model with respect to the RS model.

==> bulkfermions.tex <==
\chapter{Bulk fermions}

\label{chap:bulkfermions}

\begin{copypaste}

--- This is part of the long paper, addressing the rederivation of EWPO parameters integrating out the KK modes --- 


\subsection{Rederivation summing over KK modes}
\label{KK}

In this subsection we present very general expressions for current-current operators which result from integrating out KK gauge bosons of the 5D SM. We will then show that these dimension-six operators result in the same expressions for the precision observables obtained in Sec.~\ref{STholo}. In addition the results we derive will be useful starting points for future studies of more general models with fermions propagating in the bulk, in particular models of flavour~\cite{Agashe:2004cp,Davoudiasl:2009cd}.

Let us envisage a general gauge interaction of the form
%
\be
g_5\int d^5x \sqrt{g}\,A_M(x,y) \sum_i  J_{i}^M(x,y)\,,
\ee
%
where for clarity we have suppressed the sum over the adjoint gauge indices. The index $i$ runs over all the fermions and scalars coupling to $A_M$. Focussing on the zero modes in the currents we can write
%
\be
J^\mu_i(x,y)=y_1^{-1}e^{2A(y)}\,\omega_i(y) j_i^\mu(x)\,.
\ee
%
where the functions $\omega_i$ are defined in terms of the zero mode wave functions as
%
\be
\omega_i(y)\equiv \left\{
\begin{array}{cc}
e^{-2A}\, \xi_{i,0}^2(y)& {\rm scalars}\\
e^{-3A}\, \psi_{i,0}^2(y)& {\rm fermions}
\end{array}\right.,\qquad 
\Omega_i(y)=\frac{1}{y_1}\int_0^y\omega_i\,.
\ee
%
For later use we also have defined the integral $\Omega_i(y)$. Notice that the functions $\omega_i$ are distributions normalized to $y_1$ which implies that $\Omega_i(y_1)=1$.
We would like to integrate out the KK modes of $A_M$ to obtain the effective Lagrangian of dimension-six operators
%
\be
\mathcal L_{\rm eff}=\frac{g_5^2}{2} \sum_{i,j}\alpha_{ij} \, j^{\phantom{\mu}}_{i\,\mu}(x) j^\mu_j(x)\,.
\ee
%
In other words we would like to compute the diagrams in Fig.~\ref{diagramas}.
%
\begin{figure}[t]
\begin{center}
%\SetScale{.5}
\begin{picture}(65,80)(35,-20)
\SetWidth{1.}
\Vertex(25,25){3}
\Vertex(100,25){3}
\ArrowLine(0,50)(25,25)
\ArrowLine(25,25)(0,0)
\Photon(25,25)(100,25){3}{5}
\ArrowLine(125,50)(100,25)
\ArrowLine(100,25)(125,0)
\put(30,10){$A_M$}
\put(80,10){$A_N$}
\put(-25,20){$g_5 J_i^M$}
\put(120,20){$g_5J_j^N$}
\end{picture}
\vspace{-1cm}
\end{center}
\caption{\it Diagram contributing to the effective Lagrangian.}
\label{diagramas}
\end{figure}
%
To this end we need to evaluate 
%
\be
\alpha^{B_0B_1}_{ij}= \frac{1}{y_1^3}\int_0^{y_1}
 dy\,dy'\,\omega_i(y)\,\omega_j(y')\,G_{B_0B_1}(y,y')
\ee
%
where $G_{B_0B_1}(y,y')$ is the 5D gauge boson propagator at zero 4D momentum (with any possible zero modes subtracted). The precise definition and explicit expressions are given in App.~\ref{app:propagators}. The subscript $B_i=N,D$ denotes the type of boundary conditions of the gauge field at $y=y_i$ (Neumann or Dirichlet).
Using the results for the propagators, Eqs.~(\ref{GBB}) and (\ref{GNN}), 
one obtains (after performing suitable partial integrations)
%
\begin{align}
\alpha^{DN}_{ij}&=&\int e^{2A}\,(1-\Omega_i)(1-\Omega_j)\,,\nonumber\\
\alpha^{ND}_{ij}&=&\int e^{2A}\,\Omega_i\Omega_j\,,\nonumber\\
\alpha^{DD}_{ij}&=&\int e^{2A}\Omega_i\Omega_j-\frac{\int e^{2A}
\Omega_i\cdot\int e^{2A}\Omega_j}{\int e^{2A}}
\,,\nonumber\\
\alpha^{NN}_{ij}&=&
\int e^{2A}\,\left(\Omega_i-\frac{y}{y_1}\right)\left(\Omega_j-\frac{y}{y_1}\right)
\,.
\end{align}
%
All integrations are between $0$ and $y_1$. These remarkably simple expressions are totally general and valid for arbitrary background metric and matter zero-mode wave function.
It is straightforward to check that in case one or both of the currents are localized on the UV brane ($\Omega_i(y)=1$), $\alpha^{DN}$ and $\alpha^{DD}$ are zero. Similarly if one or both currents reside entirely on the IR brane ($\Omega_i(y)=0$) the amplitudes $\alpha^{ND}$ and $\alpha^{DD}$ vanish. Finally if $\omega_i(y)=1$ (for instance the case of $c=1/2$ for fermions in RS) one finds $\alpha^{NN}=0$. The last result can also be understood from the individual couplings between the current and each gauge KK mode, $\int \omega f_n=\int f_n$. This integral vanishes as a consequence of the orthogonality of the KK wave functions with the (flat) zero mode wave function $f_0=1$. 

Let us apply this formalism to compute the precision observables~\cite{Davoudiasl:2009cd}. Only SM gauge fields propagate in the bulk, and all of them have Neumann-Neumann BC. Imposing a light Higgs it makes sense to keep the latter in the effective theory and compute the operators involving both Higgs and fermion currents. The effective 4D Lagrangian thus reads
%
\begin{align}
\mathcal L_{\rm eff}=\mathcal L_{\rm SM}
&+&\frac{g_5^2}{2}\left(\widehat\alpha \, j_h^{L}\cdot j^L_{h} +2\widehat\beta\,  j_h^L\cdot j_f^L+\widehat\gamma\,  j_f^L\cdot j_f^L\right)\nonumber\\
&
+&\frac{g_5'^2}{2}\left( \widehat\alpha\, j_h^{Y}\cdot j^Y_{h} +2\widehat\beta\,  j_h^Y\cdot j_f^Y+\widehat\gamma\,  j_f^Y\cdot j_f^Y\right)
\end{align}
%
where $j_h^{L,Y}$ and $j_f^{L,Y}$ are the SM Higgs and fermion currents coupling to $SU(2)_L\times U(1)_Y$ gauge bosons and
%
\begin{align}
\widehat\alpha&=&\alpha_{hh}^{NN}=\int e^{2A}\,\left(\Omega_h-\frac{y}{y_1}\right)^2
,\nonumber\\
\widehat\beta&=&\alpha_{hf}^{NN}=\int e^{2A}\,\left(\Omega_h-\frac{y}{y_1}\right)\left(\Omega_f-\frac{y}{y_1}\right)\,,\nonumber\\
\widehat\gamma&=&\alpha_{ff}^{NN}=\int e^{2A}\,\left(\Omega_f-\frac{y}{y_1}\right)^2
.
\end{align}
%

For the time being we have only assumed that all fermions have the same zero mode profile which is however not necessarily localized on the UV brane. The latter case can easily be implemented by setting $\Omega_f(y)=1$. Furthermore since we are working with a light Higgs its wave function will be proportional to the background profile, see Eq.~(\ref{xiH}), and hence $\Omega_h$ coincides with $\Omega$ as defined in Eq.~(\ref{Omega}).
The assumption of ``fermion universality" implies that the effective action only depends on the "complete" fermionic currents $j_f^{L,Y}$ (as opposed to the individual quark and lepton currents) which in turn
allows one to use the gauge boson's EOM to eliminate the fermion currents from the dimension-six operators alltogether~\cite{Davoudiasl:2009cd}. This procedure leaves only the so-called ``oblique corrections"~\cite{Barbieri:2004qk} that in our case take the form~\footnote{The ellipsis denotes operators not relevant to the precision observables.}
 %
\begin{align}
\mathcal L_{\rm eff}=\mathcal L_{\rm SM}
&+&\frac{g_5'^2}{2}(\widehat\alpha-2\widehat\beta+\widehat\gamma)|H^\dagger D_\mu H|^2
+g_5g_5'(\widehat\beta-\widehat\gamma)H^\dagger W_{\mu\nu}HB^{\mu\nu}\nonumber\\
&+&\frac{\widehat\gamma y_1}{2}(\partial_\rho B_{\mu\nu})^2
+\frac{\widehat\gamma y_1}{2} (D_\rho W_{\mu\nu})^2+\dots
\end{align}
%
from which the precision observables 
%
\begin{align}
\alpha T&=&s_W^2m_Z^2y_1\int e^{2A}(\Omega_f-\Omega)^2\,,\nonumber\\
\alpha S&=&8s_W^2c_W^2 m_Z^2 y_1\int e^{2A}\left(\Omega_f-\frac{y}{y_1}\right)(\Omega_f-\Omega)\,,\nonumber\\
Y&=&c_W^2m_Z^{2}\,y_1
\int e^{2A}\left(\Omega_f-\frac{y}{y_1}\right)^2
 \,,\nonumber\\
W&=&Y\,,
\label{STYW2}
\end{align}
%
follow~\footnote{Besides the equality $Y=W$ one can also derive another relation $(\alpha S)^2\leq x (\alpha T) Y$ with $x=64 c_w^2s_w^2\approx 11.2$. This follows from Eq.~(\ref{STYW2}) by use of the Cauchy-Schwarz inequality.}. As expected these expressions reduce to Eqs.~(\ref{STYW}) in the limit of UV-brane localized fermions ($\Omega_f(y)=1$). 
One sees that with $\omega_f=1$ (the case of universal fermion bulk mass $k/2$ in RS) $S$, $W$ and $Y$ are vanishing. On the other hand $T$ is only mildly affected by this choice and does not decrease by much. In order to completely kill the $T$ parameter in RS, one would also need $a=1$ for the Higgs, which corresponds to a mostly elementary Higgs that does not solve the hierarchy problem. On the other hand one could move the fermions more towards the IR and roughly align them with the Higgs profile. In this case the $T$ parameter is suppressed, but $W$ and $Y$ can become dominant, resulting in very high bounds on the KK mass scale. In conclusion, playing with the zero mode wave functions in a pure RS background alone is not enough to reduce the bounds and a modification of the metric background is required.
\end{copypaste}

==> figs/TsobreS-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/TsobreS-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
\providecommand{\PFGstyleB}{\footnotesize}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a151}[cc][cc]{\PFGstyleB $1.5$}%
\psfrag{a1}[cc][cc]{\PFGstyleB \hspace{2mm}$1.0$}%
\psfrag{a251}[cc][cc]{\PFGstyleB $2.5$}%
\psfrag{a2}[cc][cc]{\PFGstyleB $2.0$}%
\psfrag{a351}[cc][cc]{\PFGstyleB $3.5$}%
\psfrag{a3}[cc][cc]{\PFGstyleB $3.0$}%
\psfrag{a451}[cc][cc]{\PFGstyleB $4.5$}%
\psfrag{a4}[cc][cc]{\PFGstyleB $4.0$}%
\psfrag{a5}[cc][cc]{\PFGstyleB \hspace{1mm}$0.5$}%
\psfrag{kCDelta}[bc][tc]{\PFGstyle $k\Delta$}%
\psfrag{Nu}[tc][cc]{\PFGstyle $\nu$}%
\psfrag{S111}[tc][tc]{\PFGstyle $1.1$}%
\psfrag{S11}[tc][tc]{\PFGstyle $1.0$}%
\psfrag{S121}[tc][tc]{\PFGstyle $1.2$}%
\psfrag{S5}[tc][tc]{\PFGstyle $0.5$}%
\psfrag{S6}[tc][tc]{\PFGstyle $0.6$}%
\psfrag{S7}[tc][tc]{\PFGstyle $0.7$}%
\psfrag{S8}[tc][tc]{\PFGstyle $0.8$}%
\psfrag{S9}[tc][tc]{\PFGstyle $0.9$}%
\psfrag{TSNuCDelta}[cc][bc]{\PFGstyle $\frac{T}{S} (\nu, \Delta)$}%
\psfrag{W11}[cr][cr]{\PFGstyle $1.0$}%
\psfrag{W5}[cr][cr]{\PFGstyle $0.5$}%
\psfrag{W6}[cr][cr]{\PFGstyle $0.6$}%
\psfrag{W7}[cr][cr]{\PFGstyle $0.7$}%
\psfrag{W8}[cr][cr]{\PFGstyle $0.8$}%
\psfrag{W9}[cr][cr]{\PFGstyle $0.9$}%
%

==> figs/WY-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/WY-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{kL1}[Bc][Bc]{\PFGstyle $kL_1$}%
\psfrag{S02}[tc][tc]{\PFGstyle $0.2$}%
\psfrag{S04}[tc][tc]{\PFGstyle $0.4$}%
\psfrag{S06}[tc][tc]{\PFGstyle $0.6$}%
\psfrag{S08}[tc][tc]{\PFGstyle $0.8$}%
\psfrag{S10}[tc][tc]{\PFGstyle $1.0$}%
\psfrag{W005}[cr][cr]{\PFGstyle $0.05$}%
\psfrag{W010}[cr][cr]{\PFGstyle $0.10$}%
\psfrag{W020}[cr][cr]{\PFGstyle $0.20$}%
\psfrag{W050}[cr][cr]{\PFGstyle $0.50$}%
\psfrag{W100}[cr][cr]{\PFGstyle $1.00$}%
\psfrag{W104Y104}[bc][bc]{\PFGstyle $10^4 W$}%
\psfrag{W200}[cr][cr]{\PFGstyle $2.00$}%
\psfrag{W500}[cr][cr]{\PFGstyle $5.00$}%
\psfrag{yNumberForA}[cr][cr]{\PFGstyle $0.2$}%
\psfrag{yNumberForB}[cr][cr]{\PFGstyle $0.5$}%
\psfrag{yNumberForC}[cr][cr]{\PFGstyle $1.0$}%
\psfrag{yNumberFor}[cr][cr]{\PFGstyle $0.1$}%
\psfrag{yNumberForD}[cr][cr]{\PFGstyle $2.0$}%
\psfrag{yNumberForE}[cr][cr]{\PFGstyle $5.0$}%
\psfrag{yNumberForF}[cr][cr]{\PFGstyle $10.0$}%
\psfrag{yNumberForG}[cr][cr]{\PFGstyle $20.0$}%
\psfrag{yNumberForH}[cr][cr]{\PFGstyle $50.0$}%
%


==> figs/Z-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/Z-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
\providecommand{\PFGstyleB}{\footnotesize}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a10}[cc][cc]{\PFGstyleB $10$}%
\psfrag{a12}[cc][cc]{\PFGstyleB $12$}%
\psfrag{a1}[cc][cc]{\PFGstyleB $1$}%
\psfrag{a2}[cc][cc]{\PFGstyleB $2$}%
\psfrag{a4}[cc][cc]{\PFGstyleB $4$}%
\psfrag{a6}[cc][cc]{\PFGstyleB $6$}%
\psfrag{a8}[cc][cc]{\PFGstyleB $8$}%
\psfrag{kCDelta}[bc][tc]{\PFGstyle $k\Delta$}%
\psfrag{Nu}[tc][cc]{\PFGstyle $\nu$}%
\psfrag{S11}[tc][tc]{\PFGstyle $1.0$}%
\psfrag{S5}[tc][tc]{\PFGstyle $0.5$}%
\psfrag{S6}[tc][tc]{\PFGstyle $0.6$}%
\psfrag{S7}[tc][tc]{\PFGstyle $0.7$}%
\psfrag{S8}[tc][tc]{\PFGstyle $0.8$}%
\psfrag{S9}[tc][tc]{\PFGstyle $0.9$}%
\psfrag{W11}[cr][cr]{\PFGstyle $1.0$}%
\psfrag{W5}[cr][cr]{\PFGstyle $0.5$}%
\psfrag{W6}[cr][cr]{\PFGstyle $0.6$}%
\psfrag{W7}[cr][cr]{\PFGstyle $0.7$}%
\psfrag{W8}[cr][cr]{\PFGstyle $0.8$}%
\psfrag{W9}[cr][cr]{\PFGstyle $0.9$}%
\psfrag{ZNuCDelta}[cc][bc]{\PFGstyle $Z(\nu ,\Delta )$}%
%

==> figs/a-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/a-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
\providecommand{\PFGstyleB}{\footnotesize}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a221}[cc][cc]{\PFGstyleB $2.2$}%
\psfrag{a231}[cc][cc]{\PFGstyleB $2.3$}%
\psfrag{a241}[cc][cc]{\PFGstyleB $2.4$}%
\psfrag{a261}[cc][cc]{\PFGstyleB $2.6$}%
\psfrag{a281}[cc][cc]{\PFGstyleB $2.8$}%
\psfrag{a321}[cc][cc]{\PFGstyleB $3.2$}%
\psfrag{a341}[cc][cc]{\PFGstyleB $3.4$}%
\psfrag{a3}[cc][cc]{\PFGstyleB $3.0$}%
\psfrag{aNuCDelta}[cc][bc]{\PFGstyle $a_0(\nu,\Delta)$}%
\psfrag{kCDelta}[bc][bc]{\PFGstyle $k\Delta$}%
\psfrag{Nu}[tc][cc]{\PFGstyle $\nu$}%
\psfrag{S111}[tc][tc]{\PFGstyle $1.1$}%
\psfrag{S11}[tc][tc]{\PFGstyle $1.0$}%
\psfrag{S5}[tc][tc]{\PFGstyle $0.5$}%
\psfrag{S6}[tc][tc]{\PFGstyle $0.6$}%
\psfrag{S7}[tc][tc]{\PFGstyle $0.7$}%
\psfrag{S8}[tc][tc]{\PFGstyle $0.8$}%
\psfrag{S9}[tc][tc]{\PFGstyle $0.9$}%
\psfrag{W11}[cr][cr]{\PFGstyle $1.0$}%
\psfrag{W5}[cr][cr]{\PFGstyle $0.5$}%
\psfrag{W6}[cr][cr]{\PFGstyle $0.6$}%
\psfrag{W7}[cr][cr]{\PFGstyle $0.7$}%
\psfrag{W8}[cr][cr]{\PFGstyle $0.8$}%
\psfrag{W9}[cr][cr]{\PFGstyle $0.9$}%
%

==> figs/boundsall-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/boundsall-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
\providecommand{\PFGstyleB}{\small}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{BoxmKKTeV}[tc][Bc]{\PFGstyle $m_{\mathrm{KK}}~(\mathrm{TeV})$}%
\psfrag{gauge}[cc][cc]{\PFGstyleB $\text{gauge}$}%
\psfrag{graviton}[cc][cc]{\PFGstyleB $\text{graviton}$}%
%%%\psfrag{Higgspseud}[cc][cc]{\PFGstyleB $\text{Higgs $\&$ pseudoscalar}$pseudoscalar}%
\psfrag{Higgs}[cc][cc]{\PFGstyleB $\text{Higgs}$}%
%%%\psfrag{pseudoscal}[cc][cc]{\PFGstyleB $\text{pseudoscalar}$}%
\psfrag{LBoxLAdS}[Bc][cc]{\PFGstyle $kL_1$}%
\psfrag{radion}[cc][cc]{\PFGstyleB $\text{radion}$}%
\psfrag{S2}[tc][tc]{\PFGstyle $0.2$}%
\psfrag{S3}[tc][tc]{\PFGstyle $0.3$}%
\psfrag{S4}[tc][tc]{\PFGstyle $0.4$}%
\psfrag{S5}[tc][tc]{\PFGstyle $0.5$}%
\psfrag{S6}[tc][tc]{\PFGstyle $0.6$}%
\psfrag{S7}[tc][tc]{\PFGstyle $0.7$}%
\psfrag{S8}[tc][tc]{\PFGstyle $0.8$}%
\psfrag{W0}[cr][cr]{\PFGstyle $0$}%
\psfrag{W21}[cr][cr]{\PFGstyle $2$}%
\psfrag{W41}[cr][cr]{\PFGstyle $4$}%
\psfrag{W61}[cr][cr]{\PFGstyle $6$}%
\psfrag{W81}[cr][cr]{\PFGstyle $8$}%
\psfrag{W12}[cr][cr]{\PFGstyle $10$}%
%


==> figs/boundsnu-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/boundsnu-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
\providecommand{\PFGstyleB}{\footnotesize}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{Delta01}[cl][cc]{\PFGstyle $\delta=0.1$}%
\psfrag{Delta10}[cl][cc]{\PFGstyle $\delta=1$}%
\psfrag{LLAdS}[Bc][Bc]{\PFGstyle $kL_1$}%
\psfrag{mTeV}[tc][cc]{\PFGstyle $m_{\mathrm{KK}}~(\mathrm{TeV})$}%
\psfrag{Nu}[Bc][Bc]{\PFGstyle $\nu $}%
\psfrag{S11}[tc][tc]{\PFGstyle $1.0$}%
\psfrag{S151}[tc][tc]{\PFGstyle $1.5$}%
\psfrag{S21}[tc][tc]{\PFGstyle $2.0$}%
\psfrag{S251}[tc][tc]{\PFGstyle $2.5$}%
\psfrag{S31}[tc][tc]{\PFGstyle $3.0$}%
\psfrag{S5}[tc][tc]{\PFGstyle $0.5$}%
\psfrag{W0}[cr][cr]{\PFGstyle $0$}%
\psfrag{W71}[cr][cr]{\PFGstyle $7$}%
\psfrag{W11}[cr][cr]{\PFGstyle $1$}%
\psfrag{W21}[cr][cr]{\PFGstyle $2$}%
\psfrag{W31}[cr][cr]{\PFGstyle $3$}%
\psfrag{W41}[cr][cr]{\PFGstyle $4$}%
\psfrag{W51}[cr][cr]{\PFGstyle $5$}%
\psfrag{W61}[cr][cr]{\PFGstyle $6$}%
\psfrag{a02}[cc][cc]{\PFGstyleB $0.2$}%
\psfrag{a04}[cc][cc]{\PFGstyleB $0.4$}%
\psfrag{a06}[cc][cc]{\PFGstyleB $0.6$}%
\psfrag{a08}[cc][cc]{\PFGstyleB $0.8$}%
\psfrag{a1}[cc][cc]{\PFGstyleB $1$}%
%


==> figs/ellipses-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/fig/ellipses-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
\providecommand{\PFGstyleB}{\large \sf \color{white}}%
\providecommand{\PFGstyleC}{\large \sf}%
\providecommand{\PFGstyleD}{\small \bf}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{a}[cc][cc]{\PFGstyleD (a)}%
\psfrag{b}[cc][cc]{\PFGstyleD (b)}%
\psfrag{c}[cc][cc]{\PFGstyleD (c)}%
\psfrag{d}[cc][cc]{\PFGstyleD (d)}%
\psfrag{S0}[tc][tc]{\PFGstyle $0$}%
\psfrag{S125}[tc][tc]{\PFGstyle $ $}%
\psfrag{S15}[tc][tc]{\PFGstyle $0.15$}%
\psfrag{S1}[tc][tc]{\PFGstyle $0.10$}%
\psfrag{S25m1}[tc][tc]{\PFGstyle $ $}%
\psfrag{S5m1}[tc][tc]{\PFGstyle $0.05$}%
\psfrag{S75m1}[tc][tc]{\PFGstyle $ $}%
\psfrag{Sm25m1}[tc][tc]{\PFGstyle $ $}%
\psfrag{S}[tc][tc]{\PFGstyle $S$}%
\psfrag{Style10Lar}[cr][cc]{\PFGstyle $10~\mathrm{TeV}$}%
\psfrag{Style115Ge}[cc][cc]{\PFGstyleB $\text{115 GeV}$}%
\psfrag{Style2Larg}[cr][cc]{\PFGstyle $2~\mathrm{TeV}$}%
\psfrag{Style450Ge}[cc][cc]{\PFGstyleB $\text{450 GeV}$}%
\psfrag{Style5Larg}[cr][cc]{\PFGstyle $5~\mathrm{TeV}$}%
\psfrag{Style800Ge}[cc][cc]{\PFGstyleC $\text{800 GeV}$}%
\psfrag{StylemKKTe}[cr][cc]{\PFGstyle $m_\mathrm{KK}~~~$}%
\psfrag{T}[bc][cc]{\PFGstyle $T$}%
\psfrag{W0}[cr][cr]{\PFGstyle $0$}%
\psfrag{W1}[cr][cr]{\PFGstyle $0.1$}%
\psfrag{W2}[cr][cr]{\PFGstyle $0.2$}%
\psfrag{W3}[cr][cr]{\PFGstyle $0.3$}%
\psfrag{W4}[cr][cr]{\PFGstyle $0.4$}%
\psfrag{W5}[cr][cr]{\PFGstyle $0.5$}%
%

==> figs/minbounds-psfrag.tex <==
% -- content from the PSfragPrologue option --
%auto-ignore (makes arXiv.org ignore this file)
% This file replaces labels in an EPS graphic by LaTeX macros,
% i.e. it should be accompanied by an EPS file (~/figs/minbounds-psfrag.eps). 
\def\PFGstripminus-#1{#1}%
\def\PFGshift(#1,#2)#3{\raisebox{#2}[\height][\depth]{\hbox{%
  \ifdim#1<0pt\kern#1 #3\kern\PFGstripminus#1\else\kern#1 #3\kern-#1\fi}}}%
\providecommand{\PFGstyle}{}%
% -- end of PSfragPrologue option --
%
% psfrag replacement commands
\psfrag{Delta01}[cl][cc]{\PFGstyle $\delta=0.1$}%
\psfrag{Delta10}[cl][cc]{\PFGstyle $\delta=1$}%
\psfrag{LLAdS}[Bc][Bc]{\PFGstyle $kL_1$}%
\psfrag{mfTeV}[tc][bc]{\PFGstyle $m_{\mathrm{KK}}~(\mathrm{TeV})$}%
\psfrag{S11}[tc][tc]{\PFGstyle $1.0$}%
\psfrag{S2}[tc][tc]{\PFGstyle $0.2$}%
\psfrag{S3}[tc][tc]{\PFGstyle $0.3$}%
\psfrag{S4}[tc][tc]{\PFGstyle $0.4$}%
\psfrag{S5}[tc][tc]{\PFGstyle $0.5$}%
\psfrag{S6}[tc][tc]{\PFGstyle $0.6$}%
\psfrag{S7}[tc][tc]{\PFGstyle $0.7$}%
\psfrag{S8}[tc][tc]{\PFGstyle $0.8$}%
\psfrag{S9}[tc][tc]{\PFGstyle $0.9$}%
\psfrag{S}[cc][cc]{\PFGstyle $S$}%
\psfrag{T}[cc][cc]{\PFGstyle $T$}%
\psfrag{W0}[cr][cr]{\PFGstyle $0$}%
\psfrag{W71}[cr][cr]{\PFGstyle $7$}%
\psfrag{W11}[cr][cr]{\PFGstyle $1$}%
\psfrag{W21}[cr][cr]{\PFGstyle $2$}%
\psfrag{W31}[cr][cr]{\PFGstyle $3$}%
\psfrag{W41}[cr][cr]{\PFGstyle $4$}%
\psfrag{W51}[cr][cr]{\PFGstyle $5$}%
\psfrag{W61}[cr][cr]{\PFGstyle $6$}%
%

